Song-based Classification techniques for Endangered Bird Conservation

The work presented in this paper is part of a global framework which long term goal is to design a wireless sensor network able to support the observation of a population of endangered birds. We present the first stage for which we have conducted a knowledge discovery approach on a sample of acoustical data. We use MFCC features extracted from bird songs and we exploit two knowledge discovery techniques. One that relies on clustering-based approaches, that highlights the homogeneity in the songs of the species. The other, based on predictive modeling, that demonstrates the good performances of various machine learning techniques for the identification process. The knowledge elicited provides promising results to consider a widespread study and to elicit guidelines for designing a first version of the automatic approach for data collection based on acoustic sensors.

==> section/3_1_Description.tex <==
The initial audio data or \textit{raw data} are songs of Moqueur Gorge Blanche collected in 2009 on the site of La Caravelle~\cite{CD-Chants}. 
We have extracted seven song samples.
Each song is sampled at 44.1 kHz and stored as 16-bit signed mono .wav format files.

For each sample, MFCC features have been computed with the Java framework CoMIRVA~\cite{Schedl2007} developed and maintained by Markus Schedl (see Figure~\ref{figMfcc}(a)).
In order to simplify the computation phase, we have generated an mean fingerprint for each song, by averaging the different MFCC values provided for each coefficient (see Figure~\ref{figMfcc}(b)). Thus we have a mean fingerprint vector of 20 averaged MFCC coefficients for each of the 7 songs. Each of the 20 averaged MFCC coefficients corresponds to a time window of an original song.
\\
In this way, the problem is to determine, for such a fingerprint, whether it belongs to the species or not. In other words, we would like to predict with a good accuracy that a new song occurring belongs the Moqueur Gorge Blanche.



In order to conduct classification tasks, we have completed these samples with counter-examples to obtain a training dataset of mean fingerprints obtained on other bird species.
Thus, 17 new samples have been added for bird species such as Common blackbird, Accentor, Heron, Woodcock, etc. 

Traditionally the data mining \textit{preprocessing} step is very important since choices have to be done done for preparing, cleaning and transforming the raw data that may be often noisy, imbalanced and not in the adequate format that learning algorithms requires as input. In the current study, as described just above, the original audio data are transformed to produce the dataset composed of 24 averaged MFCC fingerprints.\\
For classification problems it is necessary to label each data sample with its corresponding class. In this work we address a typical binary classification problem consisting in determining wether or not a data sample is an actual Moqueur Gorge Blanche sing ("MGB" class) or another bird specie sing ("Other" class). \textcolor{red}{In the following, the "MGB" class will be considered as the positive class while the "Other" class will be considered as negative.} As said before, the "MGB" class contains 7 samples while the "Other" contains 17 samples  from various other bird species. Our dataset is thus clearly imbalanced since there are more than twice as much "Other" samples than "MGB". 
In order to overcome the imbalance between classes in datasets, two strategies are commonly used:
\begin{enumerate}
\item assign distinct costs to class samples (usually higher costs for the
  minority class) \cite{PazzaniMMAHB94}
\item re-sample the source dataset, either by over-sampling the
  minority class and/or under-sampling the majority class \cite{KubatM97}
\end{enumerate}
We followed the second approach to create balanced training sets. We over-sampled the "MGB" class using the {\it Synthetic Minority Over-sampling Technique} (SMOTE) algorithm \cite{ChawlaBHK02} which consists in generating synthetic examples by randomly selecting points along the lines that join a minority class original sample and some of its nearest neighbors. Since this over-sampling technique is based on random prpoerties, we generated 100 extented balanced datasets (with 16 "MGB" and 17 "Others") and we will average the performances obtained on each of them in order to have statistically significant results.


==> section/3_2_Preprocessing.tex <==

%Class labeling, training set, over sampling, ...

Traditionally the data mining preprocessing step is very important since choices have to be done done for preparing, cleaning and transforming the raw data that may be often noisy, imbalanced and not in the adequate format that learning algorithms requires as input. In the current study, as described just above, the original audio data are transformed to produce the dataset composed of 24 averaged MFCC fingerprints.\\
For classification problems it is necessary to label each data sample with its corresponding class. In this work we address a typical binary classification problem consisting in determining wether or not a data sample is an actual Moqueur Gorge Blanche sing ("MGB" class) or another bird specie sing ("Other" class). \textcolor{red}{In the following, the "MGB" class will be considered as the positive class while the "Other" class will be considered as negative.} As said before, the "MGB" class contains 7 samples while the "Other" contains 17 samples  from various other bird species. Our dataset is thus clearly imbalanced since there are more than twice as much "Other" samples than "MGB". 
In order to overcome the imbalance between classes in datasets, two strategies are commonly used:
\begin{enumerate}
\item assign distinct costs to class samples (usually higher costs for the
  minority class) \cite{PazzaniMMAHB94}
\item re-sample the source dataset, either by over-sampling the
  minority class and/or under-sampling the majority class \cite{KubatM97}
\end{enumerate}
We followed the second approach to create balanced training sets. We over-sampled the "MGB" class using the {\it Synthetic Minority Over-sampling Technique} (SMOTE) algorithm \cite{ChawlaBHK02} which consists in generating synthetic examples by randomly selecting points along the lines that join a minority class original sample and some of its nearest neighbors. Since this over-sampling technique is based on random prpoerties, we generated 100 extented balanced datasets (with 16 "MGB" and 17 "Others") and we will average the performances obtained on each of them in order to have statistically significant results.

